Pareto-Optimality, Smoothness, and Stochasticity in Learning-Augmented One-Max-Search

One-max search is a classic problem in online decision-making, in which a trader acts on a sequence of revealed prices and accepts one of them irrevocably to maximise its profit. The problem has been studied both in probabilistic and in worst-case settings, notably through competitive analysis, and more recently in learning-augmented settings in which the trader has access to a prediction on the sequence. However, existing approaches either lack smoothness, or do not achieve optimal worst-case guarantees: they do not attain the best possible trade-off between the consistency and the robustness of the algorithm. We close this gap by presenting the first algorithm that simultaneously achieves both of these important objectives. Furthermore, we show how to leverage the obtained smoothness to provide an analysis of one-max search in stochastic learning-augmented settings which capture randomness in both the observed prices and the prediction.

==> sections/plan.tex <==
\vspace{1cm}



\mypar{Second draft plan -L}

\textit{Motivation}
\begin{enumerate}
    \item Progress of ML -> reconsider many existing decision algorithms.
    \item Side-information allows to improve on the worst-case bounds of classical TCS.
    \item Beyond worst-case analysis + Algorithms with predictions 
    \item So this field appears to have great potential for allowing ML to solve problems indirectly, through the combination of decision theory with existing predictions methods.
\end{enumerate}

\textit{Problem of applicability}
\begin{enumerate}
    \item The framework of algs with predictions remains deterministic + brittleness + risk-management (not uncertainty,deterministic).
    \item However many situations are modeled by stochastics (ML, spatial models/weather, fin Math etc.) which the current brittle algorithms fails to account for.
     i) Creates difficulties quantifying effective performance guarantees.
     \item Non-smooth algorithms prevents risk assessment of algs with predictions, which is essential in stochastic real-world use cases.
     \item This makes them of little practical relevance + which means it is better to not use the prediction but use the more robust method.
\end{enumerate}

\textit{Approach}: because of the diversity of stochastic environments and decision problems, establishing a unifying picture from the get-go is unrealistic. So we will take a stepping stone approach by restricting ourselves to $\OMS{}$ a highly simplified model of financial trading.  More general problems will exhibit the same core difficulties.


\textit{{\OMS{}}}:
\begin{enumerate} 
    \item a selection problem which can be viewed as the simplest representative of OE.
    \item Describe the game.
    \item OE in TCS: optimal selection, secretaries, and prophets. 
    \item OE in Finance: Stochastic modelling and market impact.
    \item Known Pareto optimal alg.
    \item The litterature review Spyros wrote goes well here
\end{enumerate}


\textit{Goal}: Design smooth optimal algorithms for ML-augmented decision-making applicable to real use-cases in stochastic environements like financial markets and introducing tools for their analysis.

\textit{Challenges}:
\begin{enumerate}
    \item performance imperative: Optimal performance (Consistency and robustness)
    \item Smooth error degradation to permit practical assessement of performances enabling practitioners to balance risk-reward with stochastics. 
    \item flexibility to analyse many different models of stochastics through general tools and analysis. Two things must be captured i) the complex relationship between the model's output and reality (prediction "goodness" via  "correlation") ii) the impact of the distributions of the two in-and-of themselves ("useful" but "bad" prediction graph, relation to non-stationarity in historic data models in finance)
\end{enumerate}



%\subsection{{\OMS{}}} 


\textit{Literature review}:
\begin{enumerate}
    \item Seminal papers du domain + diversity of contexts/applications
    \item Optimality et Pareto optimality
    \item Smoothness and brittleness/no error analysis
    \item Error measures 
    \item (?) distributional prediction/analysis in expectation and Wasserstein 
\end{enumerate}

\textit{Contributions}:
\begin{itemize}
    \item We provide a deterministic Pareto-opt smooth algorithmic family which supersedes the work of \cite{sun_online_2024}.
    \item We provide a smooth error analysis of this family as a function of a novel multiplicative error measure. This fine analysis provides a solid foundation on which it is comparatively simple to analyse the stochastic problem. We also derive additive error. [algorithm analysis]
    \item we apply the algorithm to several stochastic models which was not possible with \cite{sun_online_2024}'s algorithm. We provide two illustrative simple models in which closed-form estimates can be derived, and derive error functions as functions of distributions of the price/prediction. We also provide a worst-case analytical framework using Optimal transport.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Execution_with_predictions/Submission/figures/optimal threshold.pdf}
    \caption{Schematic representation of random prices and prediction.}
    \label{fig:thresholds and predictions}
\end{figure}

\Cref{fig:thresholds and predictions} depicts a prediction distribution centred at $\phi^*$, the optimal threshold for a \OMS{} problem with the optimal price distributed as the blue distribution. While it is apparent that the two distributions are very different, and that the prediction doesn't predict the price in any meaningful way, an algorithm which blindly follows the prediction will still perform very well. Thus, it is possible for the 

==> sections/previous-deterministic.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

In the standard setting of the \OMS{} problem, the input consists of a sequence of prices
$\prices=(\prices_i)_{i=1}^n \in [1,\ub]^n$. At each step $i \in [n]$, the algorithm must decide irrevocably  whether to accept $\prices_i$, in which it terminates with a payoff equal to this price, or proceed 
to step $i+1$. If no price has been accepted by step $n$, then then payoff defaults to 1. 

The {\em competitive ratio} of an algorithm is defined as the worst-case ratio, over all sequences, between the algorithm's payoff and the maximum price in the sequence; we denote the latter by $\price$. We say that an algorithm has {\em threshold} $\thresh$ if it accepts the first price in the sequence that is at least $\Phi$. The optimal deterministic competitive ratio is $1/\ub$ and is achieved by an algorithm with threshold $\ub$~\cite{el-yaniv_competitive_1998}.

In the learning-augmented setting, the decision-maker receives a {\em prediction} $\pred$ of the maximum price in the input $\prices$. The payoff of an algorithm $\Alg$, in this setting, is denoted by $\Alg(\prices, \pred)$. We denote by $\con(\Alg)$ and by $\rob(\Alg)$ the consistency and the robustness of the algorithm, respectively, which are defined as
\[
\con(\Alg) = \inf_{\prices} \frac{\Alg(\prices, \price)}{\price} \;,
\;
\rob(\Alg) = \inf_{\prices,y} \frac{\Alg(\prices, y)}{\price} \;.
\]
\citet{sun_online_2024} established the Pareto front of the consistency-robustness tradeoff, albeit using a different convention for the competitive ratio, namely as the worst-case ratio between the maximum price and the algorithm's payoff~\footnote{We use the convention that the competitive ratio of the maximization problem is in $(0,1]$, since it allows for a more clean derivation of the performance as a function of the prediction error.}. Translated to the inverse convention used in this paper, their results show that the Pareto front is  the curve:
\begin{align}\label{eq:pareto_optimal_front}
    \left\{
    (\con, \rob) \in [\ub^{-1/2},1]\times [\ub^{-1},\ub^{-1/2}] \; : \;
    \con \rob \ub=1 \right\}\;,
\end{align}
In~\citet{sun_online_2024}, this front is reached by a family of algorithms parameterized by $\lambda \in [0,1]$. The consistency $\con(\lambda)$ and the robustness $\rob(\lambda)$ of this family satisfy
\[
\con(\lambda) \rob(\lambda) \ub = 1 
\quad, \quad
\frac{1}{\con(\lambda)} = \frac{\lambda}{\rob(\lambda)} + 1 - \lambda\;,
\]
and are achieved by an algorithm with a certain threshold $\thresh(\lambda, \pred)$. An equivalent expression of this threshold, as a function of the parameters $\rob$, $\ub$, and $\pred$ is
\[
\thresh^0_\rob(y) = \left\{
 \begin{array}{lll}
    \rob \ub & \text{if } y \in [1,\rob \ub) \\[5pt]
     \varphi_\rob(\pred) &\text{if } \pred \in [\rob \ub, 1/\rob)\\[8pt]
     1/\rob & \text{if } \pred \in [1/\rob, \ub],
\end{array}
\right. .
\]
where 
\[
\varphi_\rob : z \mapsto \frac{\rob \ub - 1}{1 - \rob} + \frac{1 - \rob^2 \ub}{1 - \rob} \cdot \frac{z}{\rob \ub}
\]
is the line passing through the points $(\rob\ub, \rob \ub)$ and $(\ub, 1/\rob)$.
%
The Pareto-optimal threshold function $\thresh^0_\rob$ of \cite{sun_online_2024}
is represented graphically on \cref{fig:thresh_rho} (with $\rho=0$).

Beyond the consistency-robustness tradeoffs, in this work we are interested in the performance of algorithms as a function of the prediction {\em error},  defined as $\eta(\price, \pred) = |\price - \pred|$. An algorithm is called {\em smooth} if the ratio 
$\Alg(\prices,\pred)/{\price}$ is a continuous, and monotone function of the error $\eta(\price,\pred)$.




\section{Pareto-optimal, and smooth algorithms for {\OMS{}}}\label{sec: deterministic predictions}



Despite its Pareto-optimality in terms of consistency and robustness, $\thresh^0_\rob$ suffers from a significant drawback: \textit{brittleness} \cite{elenter2024overcoming}. Specifically, \citet{benomar2025tradeoffs} showed that even an arbitrarily small positive error in the prediction can cause the ratio between the payoff of \citet{sun_pareto-optimal_2021}'s algorithm and the maximum price to shift abruptly from the consistency bound to the robustness bound. This limitation greatly reduces the algorithm's practicality, as predictions in real-world scenarios are inherently imperfect, because of the stochasticity of both the prices and the prediction.

To address this issue, \citet{benomar2025tradeoffs} proposed a randomized family of algorithms designed to mitigate brittleness and ensure smoothness. Precisely, the performance of their algorithm transitions continuously from the consistency to the robustness bound as a function of the prediction error, $\eta(\price, \pred) = |\price - \pred|$. However, the consistency and robustness levels of their algorithms deviate from the Pareto-optimal curve. Additionally, because these algorithms are randomized, they provide guarantees only in expectation, making them less suitable for risk-averse decision-makers who require guarantees for every realization of the problem.

In what follows, we present a family of deterministic algorithms that achieve Pareto-optimal consistency and robustness while also being smooth. Remarkably, these algorithms overcome the limitations of previous approaches, combining their advantages without compromising on performance.

For any mapping $\thresh: [1,\ub] \to [1,\ub]$, we define the algorithm $\A_\thresh$ for \OMS{}. Given a sequence $(\prices_i)_{i=1}^n$ and a prediction $\pred$ of $\price$, the algorithm selects the first price that exceeds the threshold $\thresh(\pred)$. 
Theorem \ref{thm:thresh-pareto-optimal} below provides a characterization of all thresholds that yield Pareto-optimal levels of consistency and robustness.

\begin{restatable}{theorem}{AllParetoOptimalThresholds}\label{thm:thresh-pareto-optimal}
For any fixed level of robustness $\rob$, the set of all thresholds $\thresh: [1,\ub] \to [1,\ub]$ such that $\A_\thresh$ has robustness $\rob$ and consistency $1/\rob\ub$ is 
\begin{align*}
\SPO := \{ \thresh : [1,\ub]& \to [1,\ub] \text{ satisfying }\\
&\forall z \in [1,\ub]: \rob \ub \leq \thresh(z) \leq \frac{1}{\rob}\\
&\forall z \in [\rob \ub,\ub]: \frac{z}{\rob \ub} \leq \thresh(z) \leq z \}
\end{align*}
\end{restatable}

The constraints defining Pareto-optimal algorithms, as stated in the previous theorem, are illustrated in Figure \ref{fig:thresh_pareto_optimal}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Execution_with_predictions/Submission/figures/thresh_PO.pdf}
    \caption{All the thresholds $\thresh$ yielding a robustness of $\rob$ and a consistency of $1/\rob \ub$.\lc{ A threshold $\thresh$ is $\rob$-robust and $1/\rob\ub$-consistent if and only if its graph lies in the shaded area.}}
    \label{fig:thresh_pareto_optimal}
\end{figure}


\subsection{Smooth and Pareto-optimal algorithms}
We now turn our attention to identifying smooth algorithms within the class proved in Theorem \ref{thm:thresh-pareto-optimal}.

The analysis of \citet{benomar2025tradeoffs} reveals that the brittleness of \citet{sun_pareto-optimal_2021}'s algorithm arises from the discontinuity of the threshold $\thresh^0_\rob$ at the point $1/\rob$. This observation suggests that the smoothness of an algorithm $\A_\thresh$ is influenced by the maximum slope of the function $z \mapsto \thresh(z)$. Guided by this idea, for fixed robustness $\rob$, we study the smoothness properties of the algorithm with threshold $\thresh^1_\rob: z \mapsto \max(\rob \ub, \varphi_\rob(z))$, which minimizes the maximum slope among thresholds in $\SPO$. To further substantiate this intuition, we analyze a family of algorithms $\{\algrho\}_{\rho \in [0,1]}$, that use thresholds interpolating $\thresh^0_\rob$ of \cite{sun_pareto-optimal_2021} and $\thresh^1_\rob$. For all $\rho \in [0,1]$, $\algrho$ selects the first price exceeding the threshold $\thresh^\rho_\rob(\pred)$ defined by
\[
\left\{
 \begin{array}{lll}
    \rob \ub & \text{if } y \in [1,\rob \ub) \\[5pt]
     \varphi_\rob(y) & \text{if } \pred \in [\rob \ub, \tfrac{1}{\rob})\\
     \varphi_\rob(\tfrac{1}{\rob}) + \dfrac{\tfrac{1}{\rob} - \varphi_\rob(\tfrac{1}{\rob})}{\rho (1-\rob)} \cdot \dfrac{\pred}{\rob \ub} & \text{if } \pred \in [\tfrac{1}{\rob}, \tfrac{1}{\rob} + \rho(\ub - \tfrac{1}{\rob}))\\[8pt]
     1/\rob & \text{if } \pred \in [\tfrac{1}{\rob} + \rho(\ub - \tfrac{1}{\rob}), \ub]
\end{array}
\right. .
\]

Figure~\ref{fig:thresh_rho} illustrates the threshold $\thresh^\rho_\rob(y)$. Notably, the case $\rho = 0$ corresponds to the algorithm of \citet{sun_pareto-optimal_2021}, while at the other extreme, $\rho = 1$, we obtain the threshold $\thresh^1_\rob: z \mapsto \max(\rob \ub, \varphi_\rob(z))$.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Execution_with_predictions/Submission/figures/thresh_rho.pdf}
    \caption{The threshold functions $\thresh^\rho_r$ of $\algrho$}
    \label{fig:thresh_rho}
\end{figure}

To establish smoothness guarantees, we adopt a multiplicative prediction error measure:  
\begin{align}
    \error:(\price,\pred)\mapsto \min\left\{\frac{\price}{\pred}\,,\,\frac{\pred}{\price}\right\}\in [\ub^{-1},1]\;,
\end{align}
which better captures the nature of the 1-max search problem. A perfect prediction corresponds to $\error(\price, \pred) = 1$, while an arbitrary prediction places $\error(\price, \pred)$ within the interval $[1/\ub, 1]$.
Unlike the additive error $\additiveerror(\price, \pred) = |\price - \pred|$ used in previous works, this measure is scale-invariant and is more suitable for analyzing the competitive ratio.

\begin{restatable}{theorem}{ConsistencyRobustnessSmoothnessComplex}\label{thm: [deterministic Pareto-Optimal smooth Algorithm] consistency-robustness-smoothness complex}
The family $\{\algrho\}_{\rob, \rho}$ satisfies
\begin{equation}\label{eq: [deterministic Pareto-Optimal smooth Algorithm/ THM consistency-robustness-smoothness complex] PR bound}
\frac{\algrho(\prices, \pred)}{\price} \geq 
\max\left(
\rob, \frac{1}{\rob \ub} \error(\price,\pred)^{\smth}
\right)\;,
\end{equation}
with $\smth = \max\left(1, \frac{1}{\rho}\big(\tfrac{\ln \ub}{ \ln (\rob \ub)}-2\big)\right)$.
\end{restatable}
The smoothness described in the previous theorem is quantified by the exponent $\smth$ of $\error$. A smaller value of $\smth$ corresponds to a slower degradation of the bound, hence improved smoothness. In the limit $\rho \to 0$, the exponent $\smth$ becomes arbitrarily large, highlighting extreme sensitivity to prediction errors. In this case, even a slight imperfection in the prediction, despite being arbitrarily close to the true maximum price, results in degradation of the bound from $1/\rob \ub$ to $\rob$. On the other hand, the best smoothness is achieved when $\rho = 1$, yielding 
\[
\smth = \max\left(1, \tfrac{\ln \ub}{ \ln (\rob \ub)} - 2\right)\;.
\]

This naturally raises the question: is the smoothness guarantee in the previous result optimal, or can we design an algorithm that achieves the same levels of consistency and robustness while improving smoothness? To address this, we establish a lower bound on the smoothness achievable by any Pareto-optimal algorithm in terms of robustness and consistency.

\begin{restatable}{theorem}{LowerBoundSmoothness}\label{thm:lower-bound-smoothness}
Let $\A$ be an algorithm with robustness $\rob$ and consistency $1/\rob \ub$. Assume that $\A$ satisfies for all $\prices \in [1,\ub]^n$ and $\pred \in [1,\ub]$ that
\begin{equation}
\frac{\A(\prices, \pred)}{\price} \geq 
\max\left(
\rob, \frac{1}{\rob \ub} \error(\price,\pred)^{\smth}
\right)\;
\end{equation}
for some $\smth \in \mathbb{R}$, then necessarily $\smth \geq \tfrac{\ln \ub}{ \ln (\rob \ub)}-2$.
\end{restatable}

This lower bound shows the optimality of the exponent achieved by $\A^1_\rob$ for $\rob \leq \ub^{-2/3}$. Indeed, for a robustness level $\rob \in [\ub^{-1}, \ub^{-2/3}]$, it holds that $\tfrac{\ln \ub}{\ln (\rob \ub)} - 2 \geq 1$. Consequently, Theorem \ref{thm: [deterministic Pareto-Optimal smooth Algorithm] consistency-robustness-smoothness complex} gives
\[
\frac{\A^1_\rob(\prices, \pred)}{\price} \geq 
\max\left(
\rob, \frac{1}{\rob \ub} \error(\price,\pred)^{\tfrac{\ln \ub}{ \ln (\rob \ub)}-2}
\right)\;,
\]
which achieves the best possible exponent for $\error$, as shown in Theorem \ref{thm:lower-bound-smoothness}. 

This implies that if we consider the exponent of $\error$ as the measure of smoothness, then for $\rob \in [\ub^{-1}, \ub^{-2/3}]$, Algorithm $\A^1_\rob$ attains the triple Pareto-optimal front for consistency, robustness, and smoothness among all deterministic algorithms for \OMS{}. For $\rob \in [\ub^{-2/3}, \ub^{-1/2}]$, $\A^1_\rob$ remains smooth and Pareto-optimal for the consistency-robustness tradeoff; however, its smoothness guarantee might admit further improvement.





\subsection{}
Learning-augmented algorithms are typically parameterized by a value $\lambda \in [0,1]$, which reflects the decision-maker's degree of trust in the prediction. A simple yet effective parametrization of $\A^1_\rob$ can be achieved by setting $\rob = \ub^{-(1-\lambda/2)}$. Noting that $1/\rob \ub = \ub^{-\lambda/2}$, and $\frac{\ln \ub}{\ln (\rob \ub)} = \frac{2}{\lambda}$, this parametrization can be used in writing the results from Theorem \ref{thm: [deterministic Pareto-Optimal smooth Algorithm] consistency-robustness-smoothness complex} as
\[
\frac{\A^1_\rob(\prices, \pred)}{\price} \geq 
\max\left(
\ub^{-(1-\frac{\lambda}{2})}, \ub^{-\frac{\lambda}{2}} \error(\price,\pred)^{\max(1,\frac{2}{\lambda} - 2)}
\right)\;.
\]

An advantage of using the multiplicative error $\error$ is that the obtained bounds can be readily adapted to provide bounds on the inverse ratio $\price/\A^1_\rob(\prices,\pred)$, which is also commonly used as a definition of the competitive ratio in \OMS{} \cite{}\ltodo{missing citation}. By defining the inverse error as $\Bar{\error} = 1/\error = \max\left\{\frac{\price}{\pred}, \frac{\pred}{\price}\right\}$, we obtain
\[
\frac{\price}{\A^1_\rob(\prices, \pred)} \leq 
\min\left(
\ub^{1-\frac{\lambda}{2}}, \ub^{\frac{\lambda}{2}} \Bar{\error}(\price,\pred)^{\max(1,\frac{2}{\lambda} - 2)}
\right)\;.
\]

While the multiplicative error provides a more natural fit for the problem at hand, as discussed earlier, we also derive smoothness guarantees for $\A^1_\rob$ using the additive error $\additiveerror(\price,\pred) = |\price - \pred|$ in Appendix \ref{appendix:additive-error}.



==> sections/previous_intro.tex <==
\section{Introduction}\label{sec:introduction}


% MOTIVATION
\ltodo{imo, a bit generic} The rapid advancement of machine learning (ML) and artificial intelligence (AI) in recent years has led to the development of powerful tools capable of learning complex patterns in data and time series, facilitating high-quality predictions. However, the accuracy of these predictions is strongly influenced by factors such as the choice of the ML model, data quality, stochasticity, and various other elements.\lc{What about the decision theoretic algorithm design question (how does the prediction change behaviour)?} As a result, leveraging these predictions in decision-making processes is nontrivial. This challenge has spurred the emergence of learning-augmented algorithms, a field that has witnessed significant growth since the seminal works~\cite{DBLP:journals/jacm/LykourisV21} and~\cite{NIPS2018_8174}.

Learning-augmented algorithms use machine-learned {\em predictions} about the unknown input, and must guarantee an enhanced performance when predictions are correct (consistency), while maintaining reasonable performance for arbitrarily inaccurate predictions (robustness). Furthermore, their performance must degrade gracefully as the prediction error increases (smoothness).\ltodo{imo this hasn't been sufficiently motivated at this point} This paradigm marks a significant departure from traditional worst-case analysis, which tends to be overly pessimistic.\ltodo{unclear imo} It allows for more nuanced guarantees that go beyond the worst-case scenario, evaluating algorithm performance as a function of the prediction error.

% ONE-MAX SEARCH
This framework has found successful application in the design of online algorithms, data structures, and statistical learning algorithms. Notably, many online selection problems have been studied within this context~\cite{}, including the \OMS{} problem, which serves as a simplified model of financial trading. In this model, a trader observes a sequence of prices $(\prices_i)_{i=1}^n$ revealed online and must decide which price to accept irrevocably. The performance of the algorithm is then assessed as the worst-case ratio between its payoff and the maximal price $\lc{\price:=}\max_i \prices_i$. 

%PROBLEM OF APPLICABILITY

\citet{sun_pareto-optimal_2021} studied \OMS{} assuming that the trader is given additionally a prediction of the maximum price in the sequence.\ltodo{\OMS with a prediction of $\price$.} They
introduced an algorithm achieving Pareto-optimal levels of consistency and robustness—meaning that no other algorithm can simultaneously outperform it in both aspects. However, a key limitation of their algorithm is its brittleness \lc{its lack of smoothness. In fact this algorithm is \emph{brittle}, as demonstrated in \cite{benomar2025tradeoffs}, meaning its performance may catastrophically fail from arbitrarily small errors in the prediction of $\price$.}\ltodo{we've been talking about smoothness before, brittleness isn't introduced yet.}\cite{}, as demonstrated in \cite{benomar2025tradeoffs}, \ie its performance degrades abruptly from the consistency to the robustness bound for an arbitrarily small prediction error. This significantly limits the applicability of this algorithm in real-world scenarios, as both the quantity to predict and the prediction itself are naturally stochastic, and assuming perfectly accurate predictions is not realistic. Consequently, the only guarantee that holds in practice is the robustness bound, which is no better than the worst-case bound without predictions. \lc{Consequently, this algorithm cannot be expected to perform consistently better than ignoring the prediction.}

To address this issue, \citet{benomar2025tradeoffs} proposed a randomization of the Pareto-optimal algorithm, which introduces smoother behaviour, albeit at the cost of deviating from the consistency-robustness Pareto front. A natural question that arises is whether this deviation from the Pareto-optimal front is necessary to achieve smoothness guarantees.

%Beyond \OMS{}, having smooth algorithms in financial trading problems is essential $\ldots$ (talk a little bit about financial trading to justify the last section?)


\subsection{Contributions}
In both previous works on learning-augmented \OMS{} \cite{sun_pareto-optimal_2021, benomar2025tradeoffs}, the proposed algorithms select the first price that exceeds a threshold $\thresh(\pred)$, which depends on the prediction $\pred$ of the maximum price in the sequence.
We revisit the problem by first characterizing the class $\SPO$ of all thresholds $\thresh: [1,\ub] \to [1,\ub]$ that achieve a Pareto-optimal tradeoff between consistency and robustness.\ltodo{Do we have a decent justification for why thresholds are optimal we could put?}

Next, we focus on a specific family of thresholds within this class, generalizing the algorithm of \cite{sun_pareto-optimal_2021}. Surprisingly, all algorithms in this family not only preserve the Pareto-optimal trade-off between consistency and robustness, but also exhibit smoothness guarantees. These algorithms combine the best properties of the algorithms in \citet{sun_pareto-optimal_2021} and \citet{benomar2025tradeoffs}, without the need for any compromises.
In particular, our analysis shows that the smoothness of these algorithms is inversely proportional to the maximal slope of the corresponding threshold. Guided by this insight, we prove the smoothness induced by a specific threshold $\thresh^1_\rob$, which minimizes the maximal slope among all thresholds in the class $\SPO$.\ltodo{In thm 2.2. we give smoothness for the whole class no?}

Furthermore, we establish a lower bound on the smoothness of any Pareto-optimal algorithm, based on a particular notion of smoothness that we define in this paper. Remarkably, the lower bound matches the performance of the algorithm using the threshold $\thresh^1_\rob$ in the regimes where the robustness $\rob$ is in $[\ub^{-1}, \ub^{-2/3}]$, while there remains a gap between both for $\rob \in [\ub^{-2/3}, \ub^{-1/2}]$. This demonstrates that, in the first regime, our algorithm achieves a triple Pareto-optimal front between consistency, robustness, and smoothness.\ltodo{I think we can massively trim down these last two paragraphs about the smoothness but just saying we characterise the smoothness of this Pareto optimal family of thresholds, and we show that one of them is Pareto-optimal in all 3. I think the contributions are too detailed and it dilutes them.}

Our work is the first to prove a large class of algorithms that achieve Pareto-optimal levels of consistency and robustness in a learning-augmented problem, and also the first to establish a triple Pareto-optimal front between consistency, robustness, and smoothness.

%\zb{Rewrite paragraph(s) below.\\}
%Additionally, to emphasize on the necessity of having a smooth algorithm, we discuss how smoothness allows the obtained bound to be used in stochastic settings. More precisely, it enables the derivation of bounds that account for the coupling between the distributions of the maximum price and the prediction. We demonstrate this with examples of different distributions. Furthermore, as these bounds capture the coupling between the random variables, they can be analyzed in the worst case over the coupling, leading to an optimal transport problem. We propose a formulation for this problem and discuss it, which may provide an interesting avenue for future research.

\lc{The smoothness of our family of thresholds has a direct benefit in handling uncertain predictions. When predictions and prices are both random, we show how to derive general form bounds in expectation as a function of the distributions of predictions and prices and their \emph{coupling}. We provide complexity metrics and detailed bounds on some examples and a general analysis framework based on optimal transport.}

%\lc{Unlike prior work, our algorithmic family and analysis method allows us to use inherently uncertain predictions, for which this is a simple model. Prior work requires ad-hoc modifications (such as using the worst-case prediction from $\dpred$), our algorithm functions as-is and its analysis reveals rich performance estimates directly depending on the parameters of $\dpred$. }
%\ltodo{this par didn't fit in the main text, it should fit better in the intro or ccl, so I moved it here}

Finally, we validate our theoretical results through numerical experiments, comparing our algorithm to those from previous works and testing it in various stochastic settings.



\subsection{Related work}
\paragraph{Learning-augmented algorithms.}
The framework of learning-augmented algorithms, also known as algorithms with predictions, was introduced in \cite{}. The objective is to leverage potentially inaccurate predictions about unknown problem parameters or optimal decisions to surpass worst-case performance guarantees. This paradigm has been applied to a wide range of online algorithms within competitive analysis, including ski rental, scheduling, caching, and matching problems, among many others. Additionally, it has been employed to enhance the runtime of classical algorithms, such as sorting and graph algorithms, as well as in the design of data structures like search trees, dictionaries, and priority queues.\ltodo{I think this paragraph has a lot of redundancy with the intro. It can be skimmed down 25\%. Also, not sure about the order of related work and contributions }


\paragraph{Pareto-optimal tradeoffs.}
A key challenge in the design of learning-augmented algorithms is achieving effective tradeoffs between consistency and robustness. Numerous studies have focused on establishing Pareto-optimal tradeoffs for these competing objectives in various problems \cite{}. However, reaching the Pareto-optimal frontier can sometimes compromise smoothness. For instance, \cite{} demonstrated in the online conversion problem that any Pareto-optimal algorithm is brittle: its performance improves only with perfectly accurate predictions, while even minimal prediction errors can cause the performance to be similar to the worst-case without predictions. One proposed solution to mitigate this brittleness is the use of randomization, which enhances smoothness at the cost of degrading consistency and robustness, as demonstrated in \cite{} and \cite{} for particular problems.


\paragraph{One-Max Search} 
The one-max search problem was initially studied within the context of competitive analysis \cite{}. Assuming that all the prices are within the interval $[1,\ub]$, the optimal competitive ratio\ltodo{Hasn't been introduced before} is $1/\sqrt{\theta}$, and it is achieved by the simple strategy of selecting the first price above the threshold $\sqrt{\theta}$. The problem was revisited in the context of algorithms with predictions, where \cite{} introduced a Pareto-optimal algorithm, while \cite{} proposed a variation that ensures smoothness at the cost of deviating from the Pareto-optimal front of consistency and robustness. The design of randomized algorithms for one-max search has also been studied in the literature, and it is shown that this is equivalent to designing deterministic algorithms for the fractional version of the problem, known as the online conversion problem. In this problem, at each step $i$, the trader may choose to sell a fraction $x_i \in [0,1]$ of the asset at the current price $p_i$, under the constraint that $\sum_{i=1}^n x_i = 1$.\ltodo{Is this necessary beyond the 'fractional formulation of OMS'?} In this setting, \cite{} proved an optimal algorithm achieving a competitive ratio of $O\left(1/\log \theta\right)$, and \cite{sun_pareto-optimal_2021} also derived a Pareto-optimal optimal algorithm when given a prediction of the maximum price. Both one-max search and online conversion are specific cases of broader online selection problems, which are extensively studied due to their strong relations with financial trading and mechanism design scenarios \cite{correa_recent_2019,cartea_optimal_2015}.\ltodo{again quite a lot has already been said in the intro one page prior. I think talking about markets is of little relevance here, it makes more sense to bring it out when talking about uncertain predictions in the intro.}


\paragraph{Distributional predictions.} 
As previously discussed, a smooth algorithm is crucial in stochastic settings where both the prediction and the predicted variable are random variables. Another interesting research direction in these settings involves providing the algorithm with a predicted probability distribution \( G \), intended to approximate the true distribution \( F \)\ltodo{ I don't think these should be introduced here.} of the problem variable. This framework has been explored in the design of data structures \cite{}, where the algorithm receives predictions about the access frequencies of the stored elements. \cite{angelopoulos_contract_2024} also studied the contract scheduling problem within this framework, and more recently, \cite{dinitz_binary_2024} extended the approach to the binary search problem.

\lc{While reliability under uncertain predictions is essential for practical use-cases, smoothness is not the only approach. An alternative line of work, \emph{distributional predictions}, modifies the predictions by considering predictions of the distribution of prices rather than prices themselves. Despite recent applications of this framework to problems such as data structures \citep{}, contract scheduling \citep{angelopoulos_contract_2024}, or binary search \citep{dinitz_binary_2024}, reconciling these two lines of work remains an open question.} 








